The Parallelism Tradeoff: Limitations of Log-Precision Transformers

Despite their omnipresence in modern NLP, characterizing the computational power of transformer neural nets remains an interesting open question. We prove that transformers whose arithmetic precision is logarithmic in the number of input tokens (and whose feedforward nets are computable using space linear in their input) can be simulated by constant-depth logspace-uniform threshold circuits. This provides insight on the power of transformers using known results in complexity theory. For example, if $\mathsf L \neq \mathsf P$ (i.e., not all poly-time problems can be solved using logarithmic space), then transformers cannot even accurately solve linear equalities or check membership in an arbitrary context-free grammar with empty productions. Our result intuitively emerges from the transformer architecture's high parallelizability. We thus speculatively introduce the idea of a fundamental parallelism tradeoff: any model architecture as parallelizable as the transformer will obey limitations similar to it. Since parallelism is key to training models at massive scale, this suggests a potential inherent weakness of the scaling paradigm.

==> log-vs-practice.tex <==

\section{Log Precision vs. Practical Transformers} \label{sec:log-precision-vs-practice}

A transformer takes in $n$ tokens from a vocabulary of word pieces $\Sigma$. In practice, $n$ is often set to 512, and $\abs{\Sigma} \approx 30000$.
Thus we take $N$, the size of the problem input, to be $N = n \log \abs{\Sigma} \approx 15n$.

We can analyze under what input size $N$ the size of the circuit produced by our bound is vacuously large enough to compute any boolean function of input size $N$. Our circuit size is polynomial in $N$. A brute-force circuit to compute a function over inputs of size $N$ has size $2^N$. Thus, we can cover all inputs of size $N$ by brute force when
\begin{align*}
    N^c &\geq 2^N \\
    c \log N &\geq N .
\end{align*}
In practice, the precision of a transformer representation is $dp$, i.e., the hidden dimension times the precision of each scalar.
Setting $c \log n = dp$,
\begin{equation*}
    d \geq \frac{n \log \abs{\Sigma}}{p} .
\end{equation*}
Plugging in realistic values, we can solve for a lower bound $d_{512}$ on the hidden size under which boolean functions of input length 512 cannot be represented by a brute-force circuit:
\begin{equation*}
    d_{512}^{(32)} = \frac{512 \, \log 30000}{32} \approx 238.
\end{equation*}
assuming 32-bit arithmetic. For newer, larger language models which are trained with 16-bit arithmetic, this lower bound increases by a factor of 2 to $d_{512}^{(16)} \approx 476$ hidden dimension.

Solving instead for $n$, we can get that
\begin{equation*}
    n \leq \frac{dp}{\log \abs{\Sigma}} .
\end{equation*}
With a hidden dimension of 768 and 32-bit arithmetic, the maximum sequence length under which any boolean function can be solved by a brute-force circuit is:
\begin{align*}
    n_{768}^{(32)} &= \frac{768 \cdot 32}{\log 30000} \approx 1652 .
\end{align*}
But newer, larger language models have been trained in 16-bit arithmetic.
% https://github.com/EleutherAI/gpt-neo
% OPT, BLOOM, according to Jason Phang.
With a hidden dimension of 768 and 16-bit arithmetic, the upper bound on maximum sequence length goes down by a factor of 2, i.e., get $n_{768}^{(16)} \approx 826$.
% In practice, it is also possible to 

==> old.tex <==
\begin{align*}
    s(i, j) &= \mathbbm{1}(i \to j) \\
    h_1(i) &= \frac{1}{m_i} \sum_{j=1}^n j \mathbbm{1}(i \to j) \\
    h_2(i) &= \textrm{threshold of circuit $i$} .
\end{align*}
Where $m_i$ is the number of $j$ that $i$ connects to. 

\section{Recasting Main Result for Size-Preserving Functions}

Assume all binary operations in the transformer computation graph are size-preserving. Then prove any soft-attention transformer can be simulated in $\TC^0$.

Intuitively, say we are using exactly twice $\log N$ bits for representing non-negative unrestricted floats as $\langle a,b \rangle$ with the semantics $a 2^b$. Say we have two floats $f_1 = a_1 2^{b_1}$ and $f_2 = a_2 2^{b_2}$ with $f_1 \leq f_2$. If $f_1 < 2^{b_2}$, we have $f_1 + f_2 < (a_2 + 1) 2^{b_2}$. Since the float data type does not allow representing any number in-between $\langle a,b \rangle$ and $\langle a+1,b \rangle$, $f_1 + f_2$ will be approximated (assuming a truncation-based computation) as $a_2 2^{b_2}$, i.e., as simply $f_2$. Thus, addition of two unrestricted floats retains information about the smaller float only when they have an identical exponent term (i.e., $b_1 = b_2$), in which case the summation reduces to computing $a_1 + a_2$; if the result is larger than $N$, it's divided by $2$ (with truncation if needed) and the common exponent is increased by $1$.

The generalization to $f_1 + f_2 + \ldots f_k$ seems not obvious, though. As a difficult case, consider $a 2^b + a 2^b + a 2^{b+1} + a 2^{b+2} + \ldots + a 2^{k-2}$, which equals $a 2^{k-1}$. If $a > N/2$, the float computation (done left-to-right) will be completely lossless, it seems. In other words, full information is retained when adding these $k$ floats even though the exponents of the smallest and the largest differ by as much as $k-2$. But this also seems like a contrived case, where there are exactly right stepping stones along the way, to help retain all information.

MIGHT BE HELPFUL: Conceptually, one can view $\langle a,b \rangle$ as an $N$-bit number that is restricted to have non-zeros in only a contiguous $\log N$ size chunk, at positions $b_1, b_1+1, \ldots, b_1+\log N$.

OLD TEXT 1: For computing $f_1 + f_2$, a reasonable (truncation-based) model of addition is to right-shift $a_1$ by $b_2 - b_1$ bits, and compute the sun as $(\mathrm{RSHIFT}(a_1, b_2 - b_1) + a_2) 2^{b_2}$. Since we have only $\log N$ bits to represent the mantissa (?), the right-shift operation will result in $0$ whenever $b_2 - b_1 > \log a_1$. Thus $f_1 + f_2$ will be approximated as simply $f_2$ whenever $b_2 - b_1 > \log a_1$, i.e., $2^{b_2} > f_1$

OLD TEXT 2: If $b_2 - b_1 > \log N$, adding these two floats $f_1 + f_2$ and representing the result as $a_3 2^{b_3}$ by truncating as needed will essentially drop $f_1$ completely and end up with $f_1 + f_2 \approx f_2$. That's because $f_1 + f_2 < a_1 2^{b_2 - \log N} + f_2 \leq 2^{b_2} + f_2 = (a_2 + 1) 2^{b_2}$. (We could round things up instead of truncating, but it's the same issue.)  So exponentiation appears helpful only when $b_2 - b_1 \leq \log N$, i.e., $2^{b_2} \leq N 2^{b_1}$, i.e., $f_2 \leq N f_1 (a_2/a_1)$, i.e., $f_2 \leq N^2 f_1$.

When summing attention over $N$ floats $f_1, \ldots, f_N$, we can probably generalize this to something like $f_{\max} \leq N^2 f_{\min}$, or maybe something more subtle comes in and it goes up to $N^3$ or so. But even so, now we have numbers in a range where the min and max differ by a factor that's polynomial in $N$, so a linear embedding will hopefully (?) work out for achieving the same effect.
